Inference for bivariate extremes via a semi-parametric angular-radial model

The modelling of multivariate extreme events is important in a wide variety of applications, including flood risk analysis, metocean engineering and financial modelling. A wide variety of statistical techniques have been proposed in the literature; however, many such methods are limited in the forms of dependence they can capture, or make strong parametric assumptions about data structures. In this article, we introduce a novel inference framework for multivariate extremes based on a semi-parametric angular-radial model. This model overcomes the limitations of many existing approaches and provides a unified paradigm for assessing joint tail behaviour. Alongside inferential tools, we also introduce techniques for assessing uncertainty and goodness of fit. Our proposed technique is tested on simulated data sets alongside observed metocean time series', with results indicating generally good performance.

==> LaTeX/preamble.tex <==
%% Packages
\usepackage{setspace}
\doublespacing

\RequirePackage[dvipsnames]{xcolor}
\usepackage{amsfonts,amsmath,amssymb,mathrsfs,amsthm} % Maths mode programs
\usepackage[top=25mm, bottom=25mm, left=25mm, right=25mm]{geometry} % Page format
\usepackage{graphicx} % Figure programs
\usepackage[nodayofweek]{datetime}			
% \usepackage[authoryear,round]{natbib}
\usepackage[numbers]{natbib}

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{tkz-graph}
\usetikzlibrary{arrows}
\usepackage{colortbl}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{eso-pic}
\usepackage{bbm}
\usepackage{multirow}
\usepackage{pdflscape}
\usepackage{fancyhdr}
\usepackage{afterpage}
\usepackage{authblk}
\usepackage{chngcntr}

% FUNCTION {format.title}
% { title empty$
% { "" }
% { title }
% if$
% }

%% extra package to fix linespacing.
\usepackage{tocbasic}
\DeclareTOCStyleEntry[dynnumwidth]{tocline}{figure}% for figure entries
\DeclareTOCStyleEntry[dynnumwidth]{tocline}{table}% for table entries

%% macros
% \let\oldsection\section
% \renewcommand{\section}[1]{
% 	\setcounter{figure}{0}
% 	\setcounter{table}{0}
% 	\setcounter{equation}{0}
% 	\oldsection{#1}
% }

\counterwithin{figure}{section}

%% Table, Equation and Figure Labels
\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\renewcommand{\thetable}{\thesection.\arabic{table}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}

%% Theorem, Lemma, Proposition, Corollary
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{property}{Property}[section]

\newtheoremstyle{mystyle}  % follow `plain` defaults but change HEADSPACE.
  {}   				% ABOVESPACE
  {}   				% BELOWSPACE
  {}  				% BODYFONT
  {0pt}       		% INDENT (empty value is the same as 0pt)
  {\bfseries}	% HEADFONT
  {:}        % HEADPUNCT
  {5pt plus 1pt minus 1pt}				  % HEADSPACE. `plain` default: {5pt plus 1pt minus 1pt}
  {}          % CUSTOM-HEAD-SPEC

\theoremstyle{mystyle} % default
\newtheorem*{eg}{Working Example}

\newenvironment{workedexample}[1]{\begin{eg}\textbf{#1}\\}{\hfill $\blacktriangle$ \end{eg}}

% table environment designed to change linespacing.
% use as follows:
% \begin{MyTabular}[1.2]{ccc} % the number in the square is the linespacing
%   Standard table stuff
% \end{MyTabular}
\newenvironment{MyTabular}[2][1]
  {\def\arraystretch{#1}\tabular{#2}}
  {\endtabular}

%% title definition stuff
\makeatletter
\def\degrees#1{\gdef\@degrees{#1}}
\def\@degrees{\@latex@error{No \noexpand\degrees given}\@ehc}
\makeatother

\setcounter{secnumdepth}{3}

\def\Var{{\rm Var}\,}
\def\var{{\rm var}\,}
\def\E{{\rm E}\,}

% Ordinal Superscripts
% \newcommand{\st}{\textsuperscript{st}~}	% st superscript % commented out to avoid clash with strike-through text
\newcommand{\nd}{\textsuperscript{nd}~}	% nd superscript
\newcommand{\rd}{\textsuperscript{rd}~}	% rd superscript
\newcommand{\Th}{\textsuperscript{th}~}	% th superscript

% Maths Environments
\newenvironment{mat}{\left[ \begin{array}}{\end{array} \right]}
\newenvironment{deter}{\left| \begin{array}}{\end{array} \right|}
\newenvironment{ifbrace}{\left\{ \begin{array}}{\end{array} \right.}

% Number type
\newcommand{\NN}{\mathbb{N}}	% Natural
\newcommand{\ZZ}{\mathbb{Z}}	% Integer
\newcommand{\RR}{\mathbb{R}}	% Real

% Statistical Notation
\newcommand{\PP}[1]{\mathbb{P}\left(#1\right)}		% P()
\newcommand{\EE}[1]{\mathbb{E}\left[#1\right]}		% E[]
\newcommand{\VAR}[1]{\mbox{Var}\left(#1\right)}		% Var()
\newcommand{\PiDist}[1]{\pi\left(#1\right)}				% pi()
\newcommand{\cov}[2]{\mbox{Cov}\left(#1,#2\right)}	% Covariance
\newcommand{\corr}[2]{\mbox{Corr}\left(#1,#2\right)}	% Correlation
\newcommand{\Like}[1]{L\left(#1\right)}						% Likelihood
\newcommand{\lLike}[1]{\ell\left(#1\right)}				% log-likelihood

% Distributions
\newcommand{\Gauss}[2]{\mathcal{N}\left(\quad #1,\quad #2 \quad\right)}
\newcommand{\MVGauss}[3]{\mathcal{MVN}_{#1}\left(\quad #2,\quad #3 \quad\right)}
\newcommand{\IGam}[2]{\mathcal{IG}\left(\quad #1,\quad #2 \quad\right)}
\newcommand{\T}[4]{\mathcal{T}_{#1}\left(\quad #2, \quad #3, \quad #4 \quad \right)}
\newcommand{\dT}[5]{\mathcal{T}_{#1}\left(\quad #2; \quad #3, \quad #4, \quad #5 \quad \right)}
\newcommand{\MVT}[4]{\mathcal{T}_{#1}\left(\quad #2, \quad #3, \quad #4 \quad\right)}
\newcommand{\BETA}[2]{\mathcal{B}\mbox{eta}\left(\quad #1, \quad #2 \quad \right)}
\newcommand{\dBETA}[3]{\mathcal{B}\mbox{eta}\left(\quad #1; \quad #2, \quad #3 \quad \right)}

\newcommand{\Bern}[1]{\mathcal{B}\mbox{ern}\left(\quad #1 \quad\right)}
\newcommand{\Pois}[1]{\mathcal{P}\mbox{oisson}\left(\quad #1 \quad\right)}

% Mathematical symbols
\newcommand{\half}{\dfrac{1}{2}}												% 1/2
\newcommand{\third}{\dfrac{1}{3}}												% 1/3
\newcommand{\quarter}{\dfrac{1}{4}}											% 1/4
\newcommand{\const}{\! {\rm const.}\; }									% constant
\newcommand{\recip}[1]{\frac{1}{#1}}										% reciprocal - 1/x
\newcommand{\set}[1]{\left\{ #1 \right\} }							% {---}
\newcommand{\seq}[1]{\left( #1 \right)}									% (---)
\newcommand{\e}[1]{{\mbox{exp}}\left\{ #1 \right\}}			% exponent (text)
\newcommand{\Gamm}[1]{\Gamma\left( #1 \right)}				  % Gamma function
\newcommand{\Ind}[1]{\mathbb{I}_{\left\{#1\right\}}}		% Indicator Function
\newcommand{\Id}[1]{{I}_{#1}}														% Identity Matrix
\newcommand{\limit}[2]{\stackrel{\lim }{_{ #1 \to #2 }}}% Limit
\newcommand{\maxover}[1]{\stackrel{\max }{_{ #1 }}}			% max
\newcommand{\minover}[1]{\stackrel{\min }{_{ #1 }}}			% min
\newcommand{\OVec}{\mathbf{0}}													% Zero Vector
\newcommand{\IVec}{\mathbf{1}}													% Ones Vector

\def\CB#1{{\textcolor{Green}{[CB: #1]}}}
\def\EM#1{{\textcolor{Brown}{[EM: #1]}}}
\def\CBnew#1{{\textcolor{Cyan}{ #1}}}
\newcommand{\red}[1]{\textcolor{red}{\emph{#1}}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\atantwo}{atan2}
\newcommand{\norm}[2]{\| #1 \|_{#2}}
\DeclareMathOperator{\sgn}{\text{sgn}_*}

%% extra packages for links
\usepackage[]{hyperref} % pagebackref
% \usepackage{xcolor}
% The following removes the horrible boxes around links. 
% Feel free to change the colors or comment out.
\hypersetup{ 
    colorlinks,
    linkcolor={blue!30!black},
    citecolor={blue!30!black},
    urlcolor={blue!50!black}
}

\renewcommand\Affilfont{\small\color{black}}

% This command removes and equation numbers you do not reference with \eqref.
% Note it will remove them if you use \ref for equation referencing so be careful.
% If you want a different referencing style you should redefine \eqref to the required style.
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}

\usepackage{soul} % for text strike out \st{}

